On algorithms to find p-ordering

The concept of p-ordering for a prime p was introduced by Manjul Bhargava (in his PhD thesis) to develop a generalized factorial function over an arbitrary subset of integers. This notion of p-ordering provides a representation of polynomials modulo prime powers, and has been used to prove properties of roots sets modulo prime powers. We focus on the complexity of finding a p-ordering given a prime p, an exponent k and a subset of integers modulo p^k. Our first algorithm gives a p-ordering for set of size n in time O(nk\log p), where set is considered modulo p^k. The subsets modulo p^k can be represented succinctly using the notion of representative roots (Panayi, PhD Thesis, 1995; Dwivedi et.al, ISSAC, 2019); a natural question would be, can we find a p-ordering more efficiently given this succinct representation. Our second algorithm achieves precisely that, we give a p-ordering in time O(d^2k\log p + nk \log p + nd), where d is the size of the succinct representation and n is the required length of the p-ordering. Another contribution that we make is to compute the structure of roots sets for prime powers p^k, when k is small. The number of root sets have been given in the previous work (Dearden and Metzger, Eur. J. Comb., 1997; Maulick, J. Comb. Theory, Ser. A, 2001), we explicitly describe all the root sets for p^2, p^3 and p^4.

==> temp.tex <==
\rr{more references needed,  https://link.springer.com/article/10.1007/s10801-008-0157-9, https://www.jstor.org/stable/40587258?seq=1#metadata_info_tab_contents}
